Equilibration and Typicality in Quantum Processes

Forgetfulness is a common feature of nature. Moreover, without forgetfulness, repeatability would be impossible. Despite this, small systems constantly leak information about their state to their surroundings, and quantum mechanics tells us that this information cannot be deleted, invariably returning to influence their future behaviour. How can physical nature be forgetful if it is forbidden to forget? The results within this thesis bridge this gap between what we see in the real world and what idealised physical theories say, explaining the emergence of forgetful processes from closed quantum dynamics and allowing to quantify the rate at which memory effects become relevant.

==> acronyms.tex <==
\newacronym{syst}{\texttt{S}}{System}
\newacronym{env}{\texttt{E}}{Environment}
\newacronym{syst-env}{\texttt{SE}}{System-Environment}
\newacronym{CP}{\texttt{CP}}{Completely Positive}
\newacronym{TNI}{\texttt{TNI}}{Trace Non-Increasing}
\newacronym{TP}{\texttt{TP}}{Trace Preserving}
\newacronym{CPTP}{\texttt{CPTP}}{Completely Positive Trace Preserving}
\newacronym{CPTNI}{\texttt{CPTNI}}{Completely Positive Trace Non-Increasing}
\newacronym{POVM}{\texttt{POVM}}{Positive-Operator Valued Measure}
\newacronym{CJI}{\texttt{CJI}}{Choi-Jamio\l{}kowski isomorphism}
\newacronym{NCP}{\texttt{NCP}}{Not Completely Positive}
\newacronym{pdf}{\texttt{PDF}}{Probability Density Function}
\newacronym{syst-ancilla}{\texttt{S$\mathbf{\mathsf{\Gamma}}$}}{System-Ancilla}

\newpage
